Agent-Agnostic Centralized Training for Decentralized Multi-Agent Cooperative Driving

Active traffic management with autonomous vehicles offers the potential for reduced congestion and improved traffic flow. However, developing effective algorithms for real-world scenarios requires overcoming challenges related to infinite-horizon traffic flow and partial observability. To address these issues and further decentralize traffic management, we propose an asymmetric actor-critic model that learns decentralized cooperative driving policies for autonomous vehicles using single-agent reinforcement learning. By employing attention neural networks with masking, our approach efficiently manages real-world traffic dynamics and partial observability, eliminating the need for predefined agents or agent-specific experience buffers in multi-agent reinforcement learning. Extensive evaluations across various traffic scenarios demonstrate our method's significant potential in improving traffic flow at critical bottleneck points. Moreover, we address the challenges posed by conservative autonomous vehicle driving behaviors that adhere strictly to traffic rules, showing that our cooperative policy effectively alleviates potential slowdowns without compromising safety.

==> secs/materials/tp_table.tex <==
\begin{table*}[t]
    \vspace{5pt}
    \centering
    \begin{tabular}{lllllllllllllllll}
        \toprule
         \multirow{2}{*}{\shortstack{Controller}} & \multicolumn{4}{c}{3-way intersection} & \multicolumn{4}{c}{on-ramp} & \multicolumn{4}{c}{4-way intersection} & \multicolumn{4}{c}{lane drop} \\
         & 1000 & 1500 & 2000 & 2500 & 3000 & 3500 & 4000 & 4500 & 1000 & 1500 & 2000 & 2500 & 1500 & 2000 & 2500 & 3000 \\
        \midrule
        NC & 98.2 & 84.9 & 65.5 & 53.6 & 97.9 & 96.5 & 88.3 & 79.0 & 98.3 & 85.0 & 67.2 & 54.0 & 99.3 & 93.7 & 62.0 & 51.5 \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
        DVC-5-100 & 98.2 & 90.3 & 74.8 & 61.9 & 97.9 & 96.6 & 88.5 & 79.2 & 98.1 & 87.8 & 70.2 & 57.5 & 99.0 & 97.9 & 76.4 & 62.6 \\
        DVC-10-100 & 98.5 & 93.3 & 78.4 & 65.0 & 97.9 & 96.7 & 88.8 & 79.3 & 98.0 & \textbf{91.1} & 72.5 & 58.8 & 99.2 & 97.7 & 76.7 & 62.1 \\
        DVC-20-100 & 98.4 & 94.6 & 78.9 & 65.2 & 97.9 & 96.8 & 89.0 & 79.5 & 97.9 & 90.9 & 72.1 & 59.1 & 99.5 & 99.6 & 84.2 & 70.7 \\
        DVC-40-100 & 98.2 & 92.9 & 77.9 & 68.1 & 97.9 & 96.9 & 89.5 & 79.9 & 98.2 & 91.0 & \textbf{72.6} & 58.4 & 99.4 & 99.5 & 86.8 & 71.2 \\
        DVC-80-100 & 98.5 & \textbf{95.0} & \textbf{81.2} & 67.8 & 97.9 & \cellcolor{ForestGreen!25}{97.1} & \cellcolor{ForestGreen!25}{90.5} & \cellcolor{ForestGreen!25}{80.8} & 98.0 & 89.9 & 71.4 & 58.8 & 99.4 & 99.6 & 87.6 & 71.7 \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
        CVC-5 & 98.2 & 92.6 & 77.8 & 64.0 & 97.8 & 96.7 & 88.6 & 79.2 & 97.2 & 89.1 & 70.3 & 58.4 & 99.3 & 96.7 & 75.4 & 63.3 \\
        CVC-10 & 98.4 & 93.3 & 79.2 & 66.5 & 97.9 & 96.8 & 88.8 & 79.4 & 98.0 & 90.0 & 71.4 & 58.8 & 99.2 & 97.2 & 79.6 & 65.8 \\
        CVC-20 & 98.4 & 95.3 & 80.6 & 67.6 & 97.8 & 96.8 & 89.2 & 79.8 & 97.5 & 89.0 & 69.6 & 58.7 & 99.3 & 98.8 & 83.4 & 69.8 \\
        CVC-40 & 97.6 & 86.2 & 72.9 & 60.6 & 97.9 & \textbf{97.0} & \textbf{89.7} & 80.0 & 98.0 & 90.4 & 71.0 & 59.1 & 99.6 & 99.3 & 87.9 & 76.2 \\
        CVC-80 & 98.2 & 92.8 & 77.4 & 63.9 & 97.9 & \cellcolor{ForestGreen!25}{97.1} & \cellcolor{ForestGreen!25}{90.5} & \cellcolor{ForestGreen!25}{80.8} & 97.9 & 88.6 & 70.5 & 57.8 & 99.3 & 98.8 & 83.7 & 72.4 \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
        DVC-5-50 & 98.2 & 92.1 & 76.2 & 63.8 & 97.9 & 96.6 & 88.5 & 79.0 & 98.2 & 88.1 & 68.0 & 57.5 & 99.3 & 96.3 & 73.7 & 61.6 \\
        DVC-10-50 & 98.5 & 92.5 & 76.4 & 64.4 & 97.8 & 96.7 & 88.6 & 79.2 & 98.3 & 90.5 & 72.5 & \textbf{59.6} & 99.2 & 97.3 & 78.6 & 65.6 \\
        DVC-20-50 & 98.3 & 93.3 & 79.3 & 67.1 & 97.9 & 96.8 & 88.8 & 79.5 & 98.4 & 89.7 & 72.5 & 59.1 & 99.3 & 96.4 & 80.4 & 66.9 \\
        DVC-40-50 & 98.4 & 93.7 & 80.1 & \textbf{69.1} & 97.9 & \textbf{97.0} & \textbf{89.7} & \textbf{80.1} & 97.7 & 84.8 & 69.9 & 57.4 & 99.4 & 96.5 & 73.4 & 62.1 \\
        DVC-80-50 & 98.4 & 89.7 & 74.4 & 64.6 & 97.9 & \cellcolor{ForestGreen!25}{97.1} & \cellcolor{ForestGreen!25}{90.5} & \cellcolor{ForestGreen!25}{80.8} & 98.3 & 89.1 & 71.2 & 58.8 & 99.4 & 91.7 & 61.9 & 51.4 \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
        ITSC & 98.4 & \cellcolor{ForestGreen!25}{97.2} & \cellcolor{ForestGreen!25}{92.7} & \cellcolor{ForestGreen!25}{86.1} & - & - & - & - & 98.2 & \cellcolor{ForestGreen!25}{93.7} & \cellcolor{ForestGreen!25}{82.6} & \cellcolor{ForestGreen!25}{71.8} & 99.6 & 97.8 & 82.4 & 68.7 \\
        % ALINEA & - & - & - & - & - & - & - & - & - & - & - & - & 99.6 & 97.8 & 82.4 & 68.7 \\
        \bottomrule
    \end{tabular}
    \caption{
    Throughput comparison across different maps and traffic inputs under various control schemes. Throughput, defined as the ratio of output to input traffic flow, is computed as an average over $20$ episodes, with traffic input measured in vehicles per hour. Policy names, denoting the trained controllers, concatenate the AV penetration rate and the observation range for clarity. For instance, \textit{DVC-5-100} indicates a policy with a $5\%$ AV penetration rate and a $\qty{100}{\meter}$ observation distance. \textit{ITSC} refers to intelligent traffic signal control, employing CVTSC~\cite{yan2021courteous} with an $80\%$ AV penetration at intersections and ALINEA~\cite{vinitsky2023optimizing} for lane drops. Within congested scenarios, performances are highlighted: the highest throughput (column-wise) is marked in green background, while the second-highest is in bold.
    }
    \label{tab:tp_old}
    \vspace{-5pt}
\end{table*}

==> tables/avg_tp.tex <==
\begin{table*}[]
\tiny
\begin{tabular}{lllllllllllllllll}
\toprule
Scenario & \multicolumn{4}{c}{simpleT} & \multicolumn{4}{c}{onRamp} & \multicolumn{4}{c}{simpleX} & \multicolumn{4}{c}{laneDrop} \\
Traffic Input &    1000 &    1500 &    2000 &    2500 &    3000 &     3500 &     4000 &     4500 &    1000 &    1500 &    2000 &    2500 &     1500 &    2000 &    2500 &    3000 \\
\midrule
no         &  327.25 &  423.10 &  436.30 &  450.40 &  984.35 &  1128.60 &  1175.55 &  1187.60 &  328.55 &  424.80 &  445.45 &  448.75 &   206.80 &  260.15 &  215.30 &  214.45 \\
5          &  327.10 &  449.85 &  497.70 &  520.25 &  984.50 &  1129.80 &  1177.85 &  1191.55 &  327.85 &  439.10 &  465.45 &  477.40 &          &         &         &         \\
10         &  328.15 &  464.65 &  521.10 &  545.75 &  984.70 &  1130.70 &  1181.95 &  1192.40 &  327.30 &  455.40 &  480.20 &  488.25 &   206.75 &  271.25 &  266.30 &  258.65 \\
20         &  328.00 &  471.35 &  524.70 &  548.20 &  984.65 &  1131.70 &  1183.95 &  1195.45 &  326.50 &  454.40 &  477.65 &  491.15 &          &         &         &         \\
40         &  327.30 &  463.15 &  518.35 &  572.00 &  984.65 &  1132.65 &  1190.70 &  1202.05 &  328.00 &  454.90 &  481.45 &  485.45 &          &         &         &         \\
80         &  328.30 &  473.50 &  540.05 &  569.45 &  984.65 &  1134.70 &  1204.00 &  1215.10 &         &         &         &         &          &         &         &         \\
central 5  &  327.15 &  461.50 &  517.45 &  538.05 &         &          &          &          &         &         &         &         &          &         &         &         \\
central 10 &  327.85 &  464.95 &  526.70 &  559.20 &         &          &          &          &         &         &         &         &   206.75 &  270.10 &  276.30 &  274.20 \\
central 20 &  327.90 &  474.70 &  536.15 &  568.15 &         &          &          &          &         &         &         &         &          &         &         &         \\
central 40 &         &         &         &         &         &          &          &          &         &         &         &         &          &         &         &         \\
central 80 &         &         &         &         &         &          &          &          &         &         &         &         &          &         &         &         \\
TSC        &         &         &         &         &         &          &          &          &         &         &         &         &          &         &         &         \\
\bottomrule
\end{tabular}
    \caption{Average Throughput of different maps with different input traffic controlled by different controllers. Averaged across $20$ episodes.}
    \label{tab:all_TP}
    \vspace{-5pt}
\end{table*}

==> tables/avg_tp_over_total.tex <==
\begin{table*}[]
\begin{tabular}{lllllllllllllllll}
\toprule
Scenario & \multicolumn{4}{c}{simpleT} & \multicolumn{4}{c}{onRamp} & \multicolumn{4}{c}{simpleX} & \multicolumn{4}{c}{laneDrop} \\
Traffic Input &    1000 &  1500 &  2000 &  2500 &   3000 &  3500 &  4000 &  4500 &    1000 &  1500 &  2000 &  2500 &     1500 &  2000 &  2500 & 3000 \\
\midrule
no         &    0.98 &  0.85 &  0.66 &  0.54 &   0.98 &  0.97 &  0.88 &  0.79 &    0.98 &  0.85 &  0.67 &  0.54 &     0.41 &  0.39 &  0.26 &      \\
5          &    0.98 &  0.90 &  0.75 &  0.62 &   0.98 &  0.97 &  0.89 &  0.79 &    0.98 &  0.88 &  0.70 &  0.58 &          &       &       &      \\
10         &    0.98 &  0.93 &  0.78 &  0.65 &   0.98 &  0.97 &  0.89 &  0.79 &    0.98 &  0.91 &  0.72 &  0.59 &          &       &       &      \\
20         &    0.98 &  0.95 &  0.79 &  0.65 &   0.98 &  0.97 &  0.89 &  0.79 &    0.98 &  0.91 &  0.72 &  0.59 &          &       &       &      \\
40         &    0.98 &  0.93 &  0.78 &  0.68 &   0.98 &  0.97 &  0.89 &  0.80 &    0.98 &  0.91 &  0.73 &  0.58 &          &       &       &      \\
80         &    0.99 &  0.95 &  0.81 &  0.68 &   0.98 &  0.97 &  0.90 &  0.81 &         &       &       &       &          &       &       &      \\
central 5  &    0.98 &  0.93 &  0.78 &  0.64 &        &       &       &       &         &       &       &       &          &       &       &      \\
central 10 &    0.98 &  0.93 &  0.79 &  0.67 &        &       &       &       &         &       &       &       &          &       &       &      \\
central 20 &    0.98 &  0.95 &  0.81 &  0.68 &        &       &       &       &         &       &       &       &          &       &       &      \\
central 40 &         &       &       &       &        &       &       &       &         &       &       &       &          &       &       &      \\
central 80 &         &       &       &       &        &       &       &       &         &       &       &       &          &       &       &      \\
TSC        &         &       &       &       &        &       &       &       &         &       &       &       &          &       &       &      \\
\bottomrule
\end{tabular}

    \caption{ Average TP/(TP+nTP) of different maps with different input traffic controlled by different controllers. Averaged across $20$ episodes.}
    \label{tab:all_TP_over_total}
    \vspace{-5pt}
\end{table*}

==> tables/avg_tp_over_total_with_lanedrop.tex <==
\begin{table*}[]
\begin{tabular}{l|llll|llll|llll|llll}
\toprule
Scenario & \multicolumn{4}{c|}{simpleT} & \multicolumn{4}{c|}{onRamp} & \multicolumn{4}{c|}{simpleX} & \multicolumn{4}{c}{laneDrop} \\
Traffic Input &    1000 &  1500 &  2000 &  2500 &   3000 &  3500 &  4000 &  4500 &    1000 &  1500 &  2000 &  2500 &     1500 &  2000 &  2500 &  3000 \\
\midrule
no         &    0.98 &  0.85 &  0.66 &  0.54 &   0.98 &  0.97 &  0.88 &  0.79 &    0.98 &  0.85 &  0.67 &  0.54 &     0.41 &  0.39 &  0.26 &  0.51 \\

5          &    0.98 &  0.90 &  0.75 &  0.62 &   0.98 &  0.97 &  0.89 &  0.79 &    0.98 &  0.88 &  0.70 &  0.58 &          &       &       &       \\
10         &    0.98 &  0.93 &  0.78 &  0.65 &   0.98 &  0.97 &  0.89 &  0.79 &    0.98 &  0.91 &  0.72 &  0.59 &     0.99 &  0.98 &  0.77 &  0.62 \\
20         &    0.98 &  0.95 &  0.79 &  0.65 &   0.98 &  0.97 &  0.89 &  0.79 &    0.98 &  0.91 &  0.72 &  0.59 &          &       &       &       \\
40         &    0.98 &  0.93 &  0.78 &  0.68 &   0.98 &  0.97 &  0.89 &  0.80 &    0.98 &  0.91 &  0.73 &  0.58 &          &       &       &       \\
80         &    0.99 &  0.95 &  0.81 &  0.68 &   0.98 &  0.97 &  0.90 &  0.81 &         &       &       &       &          &       &       &       \\
central 5  &    0.98 &  0.93 &  0.78 &  0.64 &        &       &       &       &         &       &       &       &          &       &       &       \\
central 10 &    0.98 &  0.93 &  0.79 &  0.67 &        &       &       &       &         &       &       &       &     0.99 &  0.97 &  0.80 &  0.66 \\
central 20 &    0.98 &  0.95 &  0.81 &  0.68 &        &       &       &       &         &       &       &       &          &       &       &       \\
central 40 &         &       &       &       &        &       &       &       &         &       &       &       &          &       &       &       \\
central 80 &         &       &       &       &        &       &       &       &         &       &       &       &          &       &       &       \\
TSC        &         &       &       &       &        &       &       &       &         &       &       &       &          &       &       &       \\
\bottomrule
\end{tabular}


    \caption{ Average TP/(TP+nTP) of different maps with different input traffic controlled by different controllers. For MA-lanedrop: TP*3600/(500*traffic input). Averaged across $20$ episodes.}
    \label{tab:all_TP_over_total_plus_lanedrop}
    \vspace{-5pt}
\end{table*}

==> tables/avg_travel_time_not_released.tex <==
\begin{table*}[]
\scriptsize
\begin{tabular}{lllllllllllllllll}
\toprule
Scenario & \multicolumn{4}{c}{simpleT} & \multicolumn{4}{c}{onRamp} & \multicolumn{4}{c}{simpleX} & \multicolumn{4}{c}{laneDrop} \\
Traffic Input &    1000 &    1500 &    2000 &    2500 &   3000 &   3500 &    4000 &    4500 &    1000 &    1500 &    2000 &    2500 &     1500 &  2000 &  2500 & 3000 \\
\midrule
no         &   12.96 &  230.04 &  395.45 &  470.25 &  14.36 &  36.96 &  173.70 &  326.06 &   14.60 &  225.87 &  366.75 &  481.99 &     0.00 &  0.00 &  0.00 &      \\
5          &   13.91 &   86.08 &  198.71 &  289.35 &  13.99 &  34.90 &  169.04 &  321.12 &   17.88 &  122.61 &  246.69 &  325.21 &          &       &       &      \\
10         &    9.79 &   55.02 &  181.18 &  273.26 &  13.90 &  33.07 &  166.28 &  320.71 &   18.38 &   81.08 &  227.02 &  328.69 &          &       &       &      \\
20         &   10.68 &   38.75 &  157.56 &  249.09 &  13.81 &  32.43 &  164.22 &  315.96 &   21.08 &   86.66 &  235.58 &  324.93 &          &       &       &      \\
40         &   12.91 &   85.25 &  216.49 &  311.52 &  13.90 &  31.65 &  153.74 &  309.20 &   14.10 &   86.25 &  231.33 &  329.65 &          &       &       &      \\
80         &    9.61 &   40.84 &  153.24 &  265.04 &  14.19 &  29.28 &  138.95 &  294.87 &         &         &         &         &          &       &       &      \\
central 5  &   12.58 &   58.17 &  173.03 &  273.08 &        &        &         &         &         &         &         &         &          &       &       &      \\
central 10 &   10.47 &   51.55 &  170.43 &  264.14 &        &        &         &         &         &         &         &         &          &       &       &      \\
central 20 &   11.07 &   32.93 &  144.04 &  237.84 &        &        &         &         &         &         &         &         &          &       &       &      \\
central 40 &         &         &         &         &        &        &         &         &         &         &         &         &          &       &       &      \\
central 80 &         &         &         &         &        &        &         &         &         &         &         &         &          &       &       &      \\
TSC        &         &         &         &         &        &        &         &         &         &         &         &         &          &       &       &      \\
\bottomrule
\end{tabular}


    \caption{Average travel time of not released vehicles of different maps with different input traffic controlled by different controllers. Averaged across $20$ episodes.}
    \label{tab:all_travel_time_released}
    \vspace{-5pt}
\end{table*}

==> tables/avg_travel_time_released.tex <==
\begin{table*}[]
\scriptsize
\begin{tabular}{lllllllllllllllll}
\toprule
Scenario & \multicolumn{4}{c}{simpleT} & \multicolumn{4}{c}{onRamp} & \multicolumn{4}{c}{simpleX} & \multicolumn{4}{c}{laneDrop} \\
Traffic Input &    1000 &   1500 &    2000 &    2500 &   3000 &   3500 &   4000 &   4500 &    1000 &   1500 &    2000 &    2500 &     1500 &   2000 &    2500 &    3000 \\
\midrule
no         &   24.19 &  73.87 &  115.77 &  107.79 &  24.79 &  34.46 &  69.07 &  85.44 &   22.55 &  79.25 &  125.87 &  113.98 &    52.09 &  84.14 &  349.41 &  472.59 \\
5          &   23.09 &  73.77 &  149.83 &  200.85 &  24.84 &  34.01 &  69.30 &  85.54 &   23.95 &  81.25 &  163.68 &  223.73 &          &        &         &         \\
10         &   21.77 &  56.06 &  130.40 &  187.73 &  24.80 &  32.73 &  67.65 &  85.61 &   23.15 &  69.23 &  153.25 &  211.11 &    52.06 &  65.71 &  239.70 &  366.92 \\
20         &   22.19 &  50.43 &  133.35 &  199.42 &  24.52 &  32.89 &  66.85 &  85.87 &   26.23 &  75.26 &  150.07 &  210.30 &          &        &         &         \\
40         &   21.99 &  53.09 &  111.20 &  143.11 &  24.58 &  31.87 &  66.07 &  85.29 &   23.67 &  68.74 &  148.42 &  214.58 &          &        &         &         \\
80         &   21.47 &  47.43 &  114.98 &  166.74 &  24.35 &  30.78 &  62.24 &  84.83 &         &        &         &         &          &        &         &         \\
central 5  &   22.00 &  60.83 &  139.19 &  191.53 &        &        &        &        &         &        &         &         &          &        &         &         \\
central 10 &   21.88 &  56.45 &  127.68 &  181.04 &        &        &        &        &         &        &         &         &    52.06 &  69.12 &  252.54 &  387.37 \\
central 20 &   21.77 &  45.53 &  118.13 &  181.53 &        &        &        &        &         &        &         &         &          &        &         &         \\
central 40 &         &        &         &         &        &        &        &        &         &        &         &         &          &        &         &         \\
central 80 &         &        &         &         &        &        &        &        &         &        &         &         &          &        &         &         \\
TSC        &         &        &         &         &        &        &        &        &         &        &         &         &          &        &         &         \\
\bottomrule
\end{tabular}

    \caption{Average travel time of released vehicles of different maps with different input traffic controlled by different controllers. Averaged across $20$ epdisodes.}
    \label{tab:all_travel_time_released}
    \vspace{-5pt}
\end{table*}
